A Formal Approach for Tuning Stochastic Oscillators

Periodic recurrence is a prominent behavioural of many biological phenomena, including cell cycle and circadian rhythms. Although deterministic models are commonly used to represent the dynamics of periodic phenomena, it is known that they are little appropriate in the case of systems in which stochastic noise induced by small population numbers is actually responsible for periodicity. Within the stochastic modelling settings automata-based model checking approaches have proven an effective means for the analysis of oscillatory dynamics, the main idea being that of coupling a period detector automaton with a continuous-time Markov chain model of an alleged oscillator. In this paper we address a complementary aspect, i.e. that of assessing the dependency of oscillation related measure (period and amplitude) against the parameters of a stochastic oscillator. To this aim we introduce a framework which, by combining an Approximate Bayesian Computation scheme with a hybrid automata capable of quantifying how distant an instance of a stochastic oscillator is from matching a desired (average) period, leads us to identify regions of the parameter space in which oscillation with given period are highly likely. The method is demonstrated through a couple of case studies, including a model of the popular Repressilator circuit.

==> automata/lha_BufferEmptingAfterFull.tex <==
\begin{tikzpicture}[scale=.8,minimum width=1cm]
\renewcommand{\arraystretch}{.7}
   \everymath{\scriptstyle}
   
%% LOCATIONS
%\draw (-3,1.5) node[initial,left, initial text=,draw,rounded corners] (l0) { \begin{tabular}{@{}c@{}}\underline{$l_0$}\\  $\dot{t}:1$ \\ $\dot{x_1}:X_I$\end{tabular} };
\draw (-3,1.5) node[initial,left, initial text=,draw,rounded corners] (l0) { \begin{tabular}{@{}c@{}}\underline{$l_0$}\\  $\dot{t}:1$ \end{tabular} };
\draw (-0.5,1.5) node[draw,rounded corners] (l1) {\begin{tabular}{@{}c@{}}\underline{$l_1$}\\  $\dot{t_1}:1$ \end{tabular}};
\draw (2.5,1.5) node[draw,rounded corners,accepting] (l2) { \begin{tabular}{@{}c@{}}\underline{$l_2$}\end{tabular} }; %\\  $\dot{t}:1$\end{tabular} };
%\draw (-3,0) node[left, draw,rounded corners, accepting] (l2) { \begin{tabular}{@{}c@{}}\underline{$l_2$}\\  $\dot{t}:1$\end{tabular} };
%{\draw (7.5,0) node[draw,rounded corners,minimum width=1cm] (l3) {\begin{tabular}{@{}c@{}}\underline{$l_3$}\\  $\dot{t}:1$\end{tabular}};}

%% ARCS
\draw [-latex'] (l0) -- (l1) node [midway, above,sloped] {$\sharp$,$x=n_i$,$\emptyset$ };
\draw [-latex'] (l1) -- (l2) node [midway, above,sloped] {$\sharp$,$x=N$,$\emptyset$ };
\draw [-latex'] (l0) .. controls +(115:10mm) and +(75:10mm) .. (l0) node [midway ,above] { $ALL$,$\top$,$\{x:=B_i\}$ };
\draw [-latex'] (l1) .. controls +(115:10mm) and +(75:10mm) .. (l1) node [midway ,above] { $ALL$,$\top$,$\{x:=B_i\}$ };
%\draw [-latex'] (l0) .. controls +(-115:15mm) and +(-75:15mm) .. (l0) node [midway ,below] { $ALL\setminus\{R_2\}$,$t< 4$,$\emptyset$ };
%\draw [-latex'] (l1) .. controls +(270:15mm) and +(270:15mm) .. (l2) node [midway ,below,sloped] {$\sharp$,$t \geq t_1 \land d=0$, $\emptyset$ };
%\draw [-latex'] (l1) -- (l2) node [midway ,midway,sloped] {\begin{tabular}{c}$\sharp$,$t\geq t_2 \land (n> x_2 \lor x_1> n)$,\\ \\ $\{\emptyset\}$\end{tabular}};

%\draw [-latex'] (l1) .. controls +(90:10mm) and +(90:10mm) .. (l3) node [midway,above,sloped] {\begin{tabular}{c}$\sharp$,$t\leq t_1 \land (x_1> n\lor n> x_2)$,\\ $\{d:= \min(\sqrt{(t-t_1)^2+(n-x_2)^2}, \sqrt{(t-t_1)^2+(n-x_1)^2})\}$ \end{tabular}};
%\draw [-latex'] (l1) -- (l3) node [midway,above,sloped] {$\sharp$,$(x_1\leq n\leq x_2)$,$\{d:= 0\}$};
%\draw [-latex'] (l1) .. controls +(300:10mm) and +(240:10mm) .. (l3) node [midway,midway,sloped]{\begin{tabular}{c}$\sharp$,$t \geq t_1 \land (x_1> n\lor n> x_2)$,\\ \\ $\{ d:= \min(d, \min(|n-x_1|,|n-x_2|)) \}$\end{tabular} }; 

%\draw [-latex'] (l3) .. controls +(270:20mm) and +(270:20mm) .. (l1) node [midway,below,sloped]{$\text{ALL}$,$\top$,$\{ n:= x_O \}$}; 

%\draw [-latex',dashed,color=red] (l3) .. controls +(285:35mm) and +(250:30mm) .. (l2) node [midway,above,sloped]{$t \geq t_2$,$\{\varnothing\}$};

{}; 
 
\end{tikzpicture}



==> automata/lha_BufferEmptingAfterFull_T.tex <==
\begin{tikzpicture}[scale=.8,minimum width=1cm]
\renewcommand{\arraystretch}{.7}
   \everymath{\scriptstyle}
   
%% LOCATIONS
%\draw (-3,1.5) node[initial,left, initial text=,draw,rounded corners] (l0) { \begin{tabular}{@{}c@{}}\underline{$l_0$}\\  $\dot{t}:1$ \\ $\dot{x_1}:X_I$\end{tabular} };
\draw (-3,1.5) node[initial,left, initial text=,draw,rounded corners] (l0) { \begin{tabular}{@{}c@{}}\underline{$l_0$}\\  $\dot{t}:1$ \end{tabular} };
\draw (-0.5,1.5) node[draw,rounded corners] (l1) {\begin{tabular}{@{}c@{}}\underline{$l_1$}\\  $\dot{t_1}:1$ \end{tabular}};
\draw (3.2,1.5) node[draw,rounded corners,accepting] (l2) { \begin{tabular}{@{}c@{}}\underline{$l_2$}\end{tabular} }; %\\  $\dot{t}:1$\end{tabular} };
%\draw (-3,0) node[left, draw,rounded corners, accepting] (l2) { \begin{tabular}{@{}c@{}}\underline{$l_2$}\\  $\dot{t}:1$\end{tabular} };
%{\draw (7.5,0) node[draw,rounded corners,minimum width=1cm] (l3) {\begin{tabular}{@{}c@{}}\underline{$l_3$}\\  $\dot{t}:1$\end{tabular}};}

%% ARCS
\draw [-latex'] (l0) -- (l1) node [midway, above,sloped] {$\sharp$,$x=n_i$,$\emptyset$ };
\draw [-latex'] (l1) -- (l2) node [midway, above,sloped] {$\sharp$,$x=N\land t_1=T$,$\emptyset$ };
\draw [-latex'] (l0) .. controls +(115:10mm) and +(75:10mm) .. (l0) node [midway ,above] { $ALL$,$\top$,$\{x:=B_i\}$ };
\draw [-latex'] (l1) .. controls +(115:10mm) and +(75:10mm) .. (l1) node [midway ,above] { $ALL$,$\top$,$\{x:=B_i\}$ };
%\draw [-latex'] (l0) .. controls +(-115:15mm) and +(-75:15mm) .. (l0) node [midway ,below] { $ALL\setminus\{R_2\}$,$t< 4$,$\emptyset$ };
%\draw [-latex'] (l1) .. controls +(270:15mm) and +(270:15mm) .. (l2) node [midway ,below,sloped] {$\sharp$,$t \geq t_1 \land d=0$, $\emptyset$ };
%\draw [-latex'] (l1) -- (l2) node [midway ,midway,sloped] {\begin{tabular}{c}$\sharp$,$t\geq t_2 \land (n> x_2 \lor x_1> n)$,\\ \\ $\{\emptyset\}$\end{tabular}};

%\draw [-latex'] (l1) .. controls +(90:10mm) and +(90:10mm) .. (l3) node [midway,above,sloped] {\begin{tabular}{c}$\sharp$,$t\leq t_1 \land (x_1> n\lor n> x_2)$,\\ $\{d:= \min(\sqrt{(t-t_1)^2+(n-x_2)^2}, \sqrt{(t-t_1)^2+(n-x_1)^2})\}$ \end{tabular}};
%\draw [-latex'] (l1) -- (l3) node [midway,above,sloped] {$\sharp$,$(x_1\leq n\leq x_2)$,$\{d:= 0\}$};
%\draw [-latex'] (l1) .. controls +(300:10mm) and +(240:10mm) .. (l3) node [midway,midway,sloped]{\begin{tabular}{c}$\sharp$,$t \geq t_1 \land (x_1> n\lor n> x_2)$,\\ \\ $\{ d:= \min(d, \min(|n-x_1|,|n-x_2|)) \}$\end{tabular} }; 

%\draw [-latex'] (l3) .. controls +(270:20mm) and +(270:20mm) .. (l1) node [midway,below,sloped]{$\text{ALL}$,$\top$,$\{ n:= x_O \}$}; 

%\draw [-latex',dashed,color=red] (l3) .. controls +(285:35mm) and +(250:30mm) .. (l2) node [midway,above,sloped]{$t \geq t_2$,$\{\varnothing\}$};

{}; 
 
\end{tikzpicture}



==> automata/lha_MeanBufferOccupation.tex <==
\begin{tikzpicture}[scale=.8,minimum width=1cm]
\renewcommand{\arraystretch}{.7}
   \everymath{\scriptstyle}
   
%% LOCATIONS
%\draw (-3,1.5) node[initial,left, initial text=,draw,rounded corners] (l0) { \begin{tabular}{@{}c@{}}\underline{$l_0$}\\  $\dot{t}:1$ \\ $\dot{x_1}:X_I$\end{tabular} };
\draw (-3,1.5) node[initial,left, initial text=,draw,rounded corners] (l0) { \begin{tabular}{@{}c@{}}\underline{$l_0$}\\  $\dot{t}:1$\\$\dot{x_i}:B_i $ \end{tabular} };
\draw (1.5,1.5) node[draw,rounded corners,accepting] (l1) {\begin{tabular}{@{}c@{}}\underline{$l_1$}\end{tabular}};

%% ARCS
\draw [-latex'] (l0) -- (l1) node [midway, above,sloped] {$\sharp$,$t=T$,$\{x_i/=T \}$ };
\draw [-latex'] (l0) .. controls +(115:10mm) and +(75:10mm) .. (l0) node [midway ,above] { $ALL$,$t<T $,$\emptyset$ };

%\draw [-latex'] (l0) .. controls +(-115:10mm) and +(-75:10mm) .. (l0) node [midway ,below] { $\{twrkM\}$,$x< N$,$\{x++\}$ };
%\draw [-latex'] (l1) .. controls +(270:15mm) and +(270:15mm) .. (l2) node [midway ,below,sloped] {$\sharp$,$t \geq t_1 \land d=0$, $\emptyset$ };
%\draw [-latex'] (l1) -- (l2) node [midway ,midway,sloped] {\begin{tabular}{c}$\sharp$,$t\geq t_2 \land (n> x_2 \lor x_1> n)$,\\ \\ $\{\emptyset\}$\end{tabular}};

%\draw [-latex'] (l1) .. controls +(90:10mm) and +(90:10mm) .. (l3) node [midway,above,sloped] {\begin{tabular}{c}$\sharp$,$t\leq t_1 \land (x_1> n\lor n> x_2)$,\\ $\{d:= \min(\sqrt{(t-t_1)^2+(n-x_2)^2}, \sqrt{(t-t_1)^2+(n-x_1)^2})\}$ \end{tabular}};
%\draw [-latex'] (l1) -- (l3) node [midway,above,sloped] {$\sharp$,$(x_1\leq n\leq x_2)$,$\{d:= 0\}$};
%\draw [-latex'] (l1) .. controls +(300:10mm) and +(240:10mm) .. (l3) node [midway,midway,sloped]{\begin{tabular}{c}$\sharp$,$t \geq t_1 \land (x_1> n\lor n> x_2)$,\\ \\ $\{ d:= \min(d, \min(|n-x_1|,|n-x_2|)) \}$\end{tabular} }; 

%\draw [-latex'] (l3) .. controls +(270:20mm) and +(270:20mm) .. (l1) node [midway,below,sloped]{$\text{ALL}$,$\top$,$\{ n:= x_O \}$}; 

%\draw [-latex',dashed,color=red] (l3) .. controls +(285:35mm) and +(250:30mm) .. (l2) node [midway,above,sloped]{$t \geq t_2$,$\{\varnothing\}$};

{}; 
 
\end{tikzpicture}



==> automata/lha_NproducedPieces.tex <==
\begin{tikzpicture}[scale=.8,minimum width=1cm]
\renewcommand{\arraystretch}{.7}
   \everymath{\scriptstyle}
   
%% LOCATIONS
%\draw (-3,1.5) node[initial,left, initial text=,draw,rounded corners] (l0) { \begin{tabular}{@{}c@{}}\underline{$l_0$}\\  $\dot{t}:1$ \\ $\dot{x_1}:X_I$\end{tabular} };
\draw (-3,1.5) node[initial,left, initial text=,draw,rounded corners] (l0) { \begin{tabular}{@{}c@{}}\underline{$l_0$}\\  $\dot{t}:1$ \end{tabular} };
\draw (-0.5,1.5) node[draw,rounded corners,accepting] (l1) {\begin{tabular}{@{}c@{}}\underline{$l_1$}\end{tabular}};

%% ARCS
\draw [-latex'] (l0) -- (l1) node [midway, above,sloped] {$\sharp$,$x=N$,$\emptyset$ };
\draw [-latex'] (l0) .. controls +(115:10mm) and +(75:10mm) .. (l0) node [midway ,above] { $ALL\setminus\{twrkM\}$,$x< N$,$\emptyset$ };

\draw [-latex'] (l0) .. controls +(-115:10mm) and +(-75:10mm) .. (l0) node [midway ,below] { $\{twrkM\}$,$x< N$,$\{x++\}$ };
%\draw [-latex'] (l1) .. controls +(270:15mm) and +(270:15mm) .. (l2) node [midway ,below,sloped] {$\sharp$,$t \geq t_1 \land d=0$, $\emptyset$ };
%\draw [-latex'] (l1) -- (l2) node [midway ,midway,sloped] {\begin{tabular}{c}$\sharp$,$t\geq t_2 \land (n> x_2 \lor x_1> n)$,\\ \\ $\{\emptyset\}$\end{tabular}};

%\draw [-latex'] (l1) .. controls +(90:10mm) and +(90:10mm) .. (l3) node [midway,above,sloped] {\begin{tabular}{c}$\sharp$,$t\leq t_1 \land (x_1> n\lor n> x_2)$,\\ $\{d:= \min(\sqrt{(t-t_1)^2+(n-x_2)^2}, \sqrt{(t-t_1)^2+(n-x_1)^2})\}$ \end{tabular}};
%\draw [-latex'] (l1) -- (l3) node [midway,above,sloped] {$\sharp$,$(x_1\leq n\leq x_2)$,$\{d:= 0\}$};
%\draw [-latex'] (l1) .. controls +(300:10mm) and +(240:10mm) .. (l3) node [midway,midway,sloped]{\begin{tabular}{c}$\sharp$,$t \geq t_1 \land (x_1> n\lor n> x_2)$,\\ \\ $\{ d:= \min(d, \min(|n-x_1|,|n-x_2|)) \}$\end{tabular} }; 

%\draw [-latex'] (l3) .. controls +(270:20mm) and +(270:20mm) .. (l1) node [midway,below,sloped]{$\text{ALL}$,$\top$,$\{ n:= x_O \}$}; 

%\draw [-latex',dashed,color=red] (l3) .. controls +(285:35mm) and +(250:30mm) .. (l2) node [midway,above,sloped]{$t \geq t_2$,$\{\varnothing\}$};

{}; 
 
\end{tikzpicture}



==> pic/repressilator_topology.tex <==
    \begin{tikzpicture}
        \node[state] (A) {1};
        \node[state, below right=of A] (B) {2};
        \node[state, below left=of A] (C) {3};

        \path[shorten >=4pt,shorten <=4pt,line width=1.5pt,-|] (A) edge (B);
        \path[shorten >=4pt,shorten <=4pt,line width=1.5pt,-|] (B) edge (C);
        \path[shorten >=4pt,shorten <=4pt,line width=1.5pt,-|] (C) edge (A);
    \end{tikzpicture}



==> prism_tex/1slot_toy1.tex <==
\medskip
%\centering
\begin{center}
{\scriptsize
%\footnotesize
\fbox{\begin{minipage}{6in}
\begin{tabbing}
\mbox{$\prismkeyword{dtmc}$} \\


\mbox{$\prismkeyword{module} \; \prismident{ProductionLine}$} \\
\mbox{$\prismident{m1}: \; [0..1] \; \prismkeyword{init} \; \prismident{m1init};$} \\
\mbox{$\prismident{m2}: \; [0..1] \; \prismkeyword{init} \; \prismident{m2init};$} \\
\mbox{$\prismident{m3}: \; [0..1] \; \prismkeyword{init} \; \prismident{m3init};$} \\
\mbox{$\prismident{b1}: \; [0..\prismident{n1}] \; \prismkeyword{init} \; \prismident{b1init};$} \\
\mbox{$\prismident{b2}: \; [0..\prismident{n2}] \; \prismkeyword{init} \; \prismident{b2init};$} \\

\mbox{$ \; [] \; (\prismident{m1}{=}0)\&(\prismident{m2}{=}0)\&(\prismident{m3}{=}0)\&(\prismident{b1}{=}0)\&(\prismident{b2}{=}0) \; \rightarrow$} \\
\mbox{$ \;  \;  \;  \;  \;  \; (1-\prismident{r1})*(1-\prismident{r2})*(1-\prismident{r3}):\prismkeyword{true}+$} \\
\mbox{$ \;  \;  \;  \;  \;  \; (1-\prismident{r1})*(1-\prismident{r2})*\prismident{r3}:(\prismident{m3'}{=}1)+$} \\
\mbox{$ \;  \;  \;  \;  \;  \; (1-\prismident{r1})*\prismident{r2}*(1-\prismident{r3}):(\prismident{m2'}{=}1)+$} \\
\mbox{$ \;  \;  \;  \;  \;  \; (1-\prismident{r1})*\prismident{r2}*\prismident{r3}:(\prismident{m2'}{=}1)\&(\prismident{m3'}{=}1)+$} \\
\mbox{$ \;  \;  \;  \;  \;  \; \prismident{r1}*(1-\prismident{r2})*(1-\prismident{r3}):(\prismident{m1'}{=}1)\&(\prismident{b1'}{=}\prismident{b1}+1)+$} \\
\mbox{$ \;  \;  \;  \;  \;  \; \prismident{r1}*(1-\prismident{r2})*\prismident{r3}:(\prismident{m1'}{=}1)\&(\prismident{m3'}{=}1)\&(\prismident{b1'}{=}\prismident{b1}+1)+$} \\
\mbox{$ \;  \;  \;  \;  \;  \; \prismident{r1}*\prismident{r2}*(1-\prismident{r3}):(\prismident{m1'}{=}1)\&(\prismident{m2'}{=}1)\&(\prismident{b1'}{=}\prismident{b1}+1)+$} \\
\mbox{$ \;  \;  \;  \;  \;  \; \prismident{r1}*\prismident{r2}*\prismident{r3}:(\prismident{m1'}{=}1)\&(\prismident{m2'}{=}1)\&(\prismident{m3'}{=}1)\&(\prismident{b1'}{=}\prismident{b1}+1);$} \\
\mbox{$ \; [] \; (\prismident{m1}{=}0)\&(\prismident{m2}{=}0)\&(\prismident{m3}{=}0)\&(\prismident{b1}{=}0)\&(0{<}\prismident{b2})\&(\prismident{b2}{<}\prismident{n2}) \; \rightarrow$} \\
\mbox{$ \;  \;  \;  \;  \;  \; (1-\prismident{r1})*(1-\prismident{r2})*(1-\prismident{r3}):\prismkeyword{true}+$} \\
\mbox{$ \;  \;  \;  \;  \;  \; (1-\prismident{r1})*(1-\prismident{r2})*\prismident{r3}:(\prismident{m3'}{=}1)\&(\prismident{b2'}{=}\prismident{b2}-1)+$} \\
\mbox{$ \;  \;  \;  \;  \;  \; (1-\prismident{r1})*\prismident{r2}*(1-\prismident{r3}):(\prismident{m2'}{=}1)+$} \\
\mbox{$ \;  \;  \;  \;  \;  \; (1-\prismident{r1})*\prismident{r2}*\prismident{r3}:(\prismident{m2'}{=}1)\&(\prismident{m3'}{=}1)\&(\prismident{b2'}{=}\prismident{b2}-1)+$} \\
\mbox{$ \;  \;  \;  \;  \;  \; \prismident{r1}*(1-\prismident{r2})*(1-\prismident{r3}):(\prismident{m1'}{=}1)\&(\prismident{b1'}{=}\prismident{b1}+1)+$} \\
\mbox{$ \;  \;  \;  \;  \;  \; \prismident{r1}*(1-\prismident{r2})*\prismident{r3}:(\prismident{m1'}{=}1)\&(\prismident{m3'}{=}1)\&(\prismident{b1'}{=}\prismident{b1}+1)\&(\prismident{b2'}{=}\prismident{b2}-1)+$} \\
\mbox{$ \;  \;  \;  \;  \;  \; \prismident{r1}*\prismident{r2}*(1-\prismident{r3}):(\prismident{m1'}{=}1)\&(\prismident{m2'}{=}1)\&(\prismident{b1'}{=}\prismident{b1}+1)+$} \\
\mbox{$ \;  \;  \;  \;  \;  \; \prismident{r1}*\prismident{r2}*\prismident{r3}:(\prismident{m1'}{=}1)\&(\prismident{m2'}{=}1)\&(\prismident{m3'}{=}1)\&(\prismident{b1'}{=}\prismident{b1}+1)\&(\prismident{b2'}{=}\prismident{b2}-1);$} \\
\mbox{$ \; [] \; (\prismident{m1}{=}0)\&(\prismident{m2}{=}0)\&(\prismident{m3}{=}0)\&(\prismident{b1}{=}0)\&(\prismident{b2}{=}\prismident{n2}) \; \rightarrow$} \\
... \\
\mbox{$\prismkeyword{module}$}

\end{tabbing}
\end{minipage}
}}
\end{center}
\medskip


==> prism_tex/2slot_toy1.tex <==
\medskip
%\centering
\begin{center}
{\scriptsize
%\footnotesize
\fbox{\begin{minipage}{6in}
\begin{tabbing}
\mbox{$\prismkeyword{dtmc}$} \\

\mbox{$\prismkeyword{global}$} \prismident{b0}:[0..\prismident{1}] \prismkeyword{init} 1; \prismcomment{// fictitious start buffer}\\
\mbox{$\prismkeyword{global}$} \prismident{b3}:[0..\prismident{1}] \prismkeyword{init} 1; \prismcomment{// fictitious end buffer} \\
%\mbox{$\prismkeyword{const} \; \prismkeyword{double} \; \prismident{p1}{=}0.01; \;  \; \prismcomment{// fail probability of machine1 }$} \\
%\mbox{$\prismkeyword{const} \; \prismkeyword{double} \; \prismident{p2}{=}0.05; \;  \; \prismcomment{// fail probability of machine2 }$} \\
%\mbox{$\prismkeyword{const} \; \prismkeyword{double} \; \prismident{p3}{=}0.02; \;  \; \prismcomment{// fail probability of machine3 }$} \\
%\mbox{$\prismkeyword{const} \; \prismkeyword{double} \; \prismident{r1}{=}0.1; \;  \; \prismcomment{// repair probability of machine1 }$} \\
%\mbox{$\prismkeyword{const} \; \prismkeyword{double} \; \prismident{r2}{=}0.2; \;  \; \prismcomment{// repair probability of machine2 }$} \\
%\mbox{$\prismkeyword{const} \; \prismkeyword{double} \; \prismident{r3}{=}0.15; \;  \; \prismcomment{// repair probability of machine3 }$} \\
%\mbox{$\prismkeyword{const} \; \prismkeyword{int} \; \prismident{n0}{=}2; \;  \; \prismcomment{// capacity of fictitious buffer zero is set to 2 }$} \\
%\mbox{$\prismkeyword{const} \; \prismkeyword{int} \; \prismident{n1}{=}8; \;  \; \prismcomment{// capacity of buffer 1 }$} \\
%\mbox{$\prismkeyword{const} \; \prismkeyword{int} \; \prismident{n2}{=}5; \;  \; \prismcomment{// capacity of buffer 2 }$} \\
%\mbox{$\prismkeyword{const} \; \prismkeyword{int} \; \prismident{n3}{=}2; \;  \; \prismcomment{// capacity of fictitious last buffer is set to 2 }$} \\
%\mbox{$\prismkeyword{const} \; \prismkeyword{int} \; \prismident{m1init}{=}1; \;  \; \prismcomment{// initial state of machine 1 }$} \\
%\mbox{$\prismkeyword{const} \; \prismkeyword{int} \; \prismident{m2init}{=}1; \;  \; \prismcomment{// initial state of machine 2 }$} \\
%\mbox{$\prismkeyword{const} \; \prismkeyword{int} \; \prismident{m3init}{=}0; \;  \; \prismcomment{// initial state of machine 3 }$} \\
%\mbox{$\prismkeyword{const} \; \prismkeyword{int} \; \prismident{b1init}{=}1; \;  \; \prismcomment{// initial state of buffer 4 }$} \\
%\mbox{$\prismkeyword{const} \; \prismkeyword{int} \; \prismident{b2init}{=}4; \;  \; \prismcomment{// initial state of buffer 5 }$} \\

\mbox{$\prismkeyword{module} \; \prismident{Phase}$} \\
\mbox{$\prismident{ph} \; : \; [1..2] \; \prismkeyword{init} \; 1;$} \\
\mbox{$[\prismident{tic}] \; \prismident{ph}{=}1 \; \rightarrow \; 1:(\prismident{ph'}{=}2);$} \prismcomment{// first slot: update machines state}\\
\mbox{$[\prismident{toc}] \; \prismident{ph}{=}2 \; \rightarrow \; 1:(\prismident{ph'}{=}1);$} \prismcomment{// second slot: update  buffer state }\\
\mbox{$\prismkeyword{endmodule}$} \\

\mbox{$\prismkeyword{module} \; \prismident{M1} \; \prismcomment{// intermediate machine, b0: upstream buffer, b1: downstream buffer}$} \\
\mbox{$ \;  \; \prismident{m1} \; : \; [0..1] \; \prismkeyword{init} \; \prismident{m1init};$} \\
\mbox{$ \;  \; [\prismident{tic}] \; \prismident{m1}{=}1    \rightarrow \prismident{p1}:(\prismident{m1'}  {=}  (\prismident{b1}{=}\prismident{n1}  |  \prismident{b0}{=}0)  ?  1  :  0)  + (1-\prismident{p1}):(\prismident{m1'}{=}1);$} \\
\mbox{$ \;  \; [\prismident{toc}] \; \prismkeyword{true} \; \rightarrow \; 1:\prismkeyword{true};$} \\
\mbox{$ \;  \; [\prismident{tic}] \; \prismident{m1}{=}0 \;  \;  \; \rightarrow \; \prismident{r1}:(\prismident{m1'}{=}1) \; + \; (1-\prismident{r1}):(\prismident{m1'}{=}0); \;  \; $} \\
\mbox{$\prismkeyword{endmodule}$} \\

\mbox{$\prismkeyword{module} \; \prismident{B1} \; \prismcomment{// intermediate buffer, m1: upstream machine, m2: downstream machine, }$} \\
\mbox{$ \;  \; \prismident{b1} \; : \; [0..\prismident{n1}] \; \prismkeyword{init} \; \prismident{b1init}; \; $} \\


\mbox{$ \;  \; [\prismident{tic}] \; \prismkeyword{true} \; \rightarrow \; 1:\prismkeyword{true};$} \\
\mbox{$ \;  \; [\prismident{toc}] \; ((\prismident{m1}{=}1 \; \& \; \prismident{b0}{>}0 \; \& \; \prismident{b1}{<}\prismident{n1}) \; \& \; !(\prismident{m2}{=}1 \; \& \; \prismident{b1}{>}0 \; \& \; \prismident{b2}{<}\prismident{n2})) \; \rightarrow \\ \; \; \; 1:(\prismident{b1'}{=}\prismident{b1}+1); \; $} \\

\mbox{$ \;  \; [\prismident{toc}] \; (!(\prismident{m1}{=}1 \; \& \; \prismident{b0}{>}0 \; \& \; \prismident{b1}{<}\prismident{n1}) \; \& \; (\prismident{m2}{=}1 \; \& \; \prismident{b1}{>}0 \; \& \; \prismident{b2}{<}\prismident{n2})) \; \rightarrow$} \\ \; \; \mbox{$1:(\prismident{b1'}{=}\prismident{b1}-1); \; \prismcomment{// decrease buffer occupation}$} \\

\mbox{$ \;  \; [\prismident{toc}] \; ( \; (!(\prismident{m1}{=}1 \; \& \; \prismident{b0}{>}0 \; \& \; \prismident{b1}{<}\prismident{n1}) \; \& \; !(\prismident{m2}{=}1 \; \& \; \prismident{b1}{>}0 \; \& \; \prismident{b2}{<}\prismident{n2})) \; |$} \\

\mbox{$ \;  \;  \;  \;  \;  \;  \;  \;  \;  \;  \; ((\prismident{m1}{=}1 \; \& \; \prismident{b0}{>}0 \; \& \; \prismident{b1}{<}\prismident{n1}) \; \& \; (\prismident{m2}{=}1 \; \& \; \prismident{b1}{>}0 \; \& \; \prismident{b2}{<}\prismident{n2})) \; ) \; \rightarrow$} \\ \; \; \; \; \; \; \; \; \;  \mbox{$1:(\prismident{b1'}{=}\prismident{b1}); \; \prismcomment{// buffer unchanged}$} \\

\mbox{$\prismkeyword{endmodule}$} \\

\mbox{$\prismkeyword{module} \; \prismident{M2}{=} \; \prismident{M1}[\prismident{m1}{=}\prismident{m2}, \; \prismident{b0}{=}\prismident{b1}, \; \prismident{b1}{=}\prismident{b2}, \; \prismident{p1}{=}\prismident{p2}, \; \prismident{r1}{=}\prismident{r2}, \; \prismident{n1}{=}\prismident{n2}, \; \\ \; \; \prismident{m1init}{=}\prismident{m2init}]$} \; \\ \mbox{$\prismkeyword{endmodule} \; $} \\
\mbox{$\prismkeyword{module} \; \prismident{B2}{=} \; \prismident{B1}[\prismident{b1}{=}\prismident{b2}, \; \prismident{m1}{=}\prismident{m2}, \; \prismident{m2}{=}\prismident{m3}, \; \prismident{b0}{=}\prismident{b1}, \; \prismident{b2}{=}\prismident{b3}, \; \prismident{n1}{=}\prismident{n2}, \; \prismident{n2}{=}\prismident{n3},$} \\ \; \; \mbox{$\prismident{b1init}{=}\prismident{b2init}] \; \\ \prismkeyword{endmodule} \; $} \\
\mbox{$\prismkeyword{module} \; \prismident{M3}{=} \; \prismident{M2}[\prismident{m2}{=}\prismident{m3}, \; \prismident{b1}{=}\prismident{b2}, \; \prismident{b2}{=}\prismident{b3}, \; \prismident{p2}{=}\prismident{p3}, \; \prismident{r2}{=}\prismident{r3}, \; \prismident{n2}{=}\prismident{n3}, \; \\ \; \; \prismident{m2init}{=}\prismident{m3init}]$} \; \\ \mbox{$\prismkeyword{endmodule} \; $} 
\end{tabbing}
\end{minipage}
}
\end{center}
\medskip


==> prism_tex/2slot_toy2.tex <==
\medskip
%\centering
\begin{center}
{\scriptsize
%\footnotesize
\fbox{\begin{minipage}{6in}
\begin{tabbing}
\mbox{$\prismkeyword{dtmc}$} \\

\mbox{$\prismkeyword{global}$} \prismident{b0}:[0..\prismident{1}] \prismkeyword{init} 1; \prismcomment{// fictitious start buffer}\\
\mbox{$\prismkeyword{global}$} \prismident{b3}:[0..\prismident{1}] \prismkeyword{init} 1; \prismcomment{// fictitious end buffer} \\

\mbox{$\prismkeyword{module} \; \prismident{Phase}$} \\
\mbox{$\prismident{ph} \; : \; [1..2] \; \prismkeyword{init} \; 1;$} \\
\mbox{$[\prismident{tic}] \; \prismident{ph}{=}1 \; \rightarrow \; 1:(\prismident{ph'}{=}2);$} \prismcomment{// first slot: update machines state}\\
\mbox{$[\prismident{toc}] \; \prismident{ph}{=}2 \; \rightarrow \; 1:(\prismident{ph'}{=}1);$} \prismcomment{// second slot: update  buffer state }\\
\mbox{$\prismkeyword{endmodule}$} \\

\mbox{$\prismkeyword{module} \; \prismident{M1} \; \prismcomment{// intermediate machine, b0: upstream buffer, b1: downstream buffer}$} \\
\mbox{$ \;  \; \prismident{m1} \; : \; [0..1] \; \prismkeyword{init} \; \prismident{m1init};$} \\
\mbox{$ \;  \; [\prismident{tic}] \; \prismident{m1}{=}1    \rightarrow \prismident{p1}:(\prismident{m1'}  {=}  (\prismident{b1}{=}\prismident{n1}  |  \prismident{b0}{=}0)  ?  1  :  0)  + (1-\prismident{p1}):(\prismident{m1'}{=}1);$} \\
\mbox{$ \;  \; [\prismident{tic}] \; \prismident{m1}{=}0 \;  \;  \; \rightarrow \; \prismident{r1}:(\prismident{m1'}{=}1) \; + \; (1-\prismident{r1}):(\prismident{m1'}{=}0); \;  \; $} \\
\mbox{$ \;  \; [\prismident{toc}] \; \prismkeyword{true} \; \rightarrow \; 1:\prismkeyword{true};$} \\
\mbox{$\prismkeyword{endmodule}$} \\

\mbox{$\prismkeyword{module} \; \prismident{B1} \; \prismcomment{// intermediate buffer, m1: upstream machine, m2: downstream machine, }$} \\
\mbox{$ \;  \; \prismident{b1} \; : \; [0..\prismident{n1}] \; \prismkeyword{init} \; \prismident{b1init}; \; $} \\


\mbox{$ \;  \; [\prismident{tic}] \; \prismkeyword{true} \; \rightarrow \; 1:\prismkeyword{true};$} \\

\mbox{$ \;  \; [\prismident{toc}] \; ((\prismident{m1}{=}1 \; \& \; \prismident{b0}{>}0 \; \& \; \prismident{b1}{<}\prismident{n1}) \; \& \; !(\prismident{m2}{=}1 \; \& \; \prismident{b1}{>}0 \; \& \; \prismident{b2}{<}\prismident{n2})) \; \rightarrow \; $}\\  \; \; \ ; \; \mbox{$ 1:(\prismident{b1'}{=}\prismident{b1}+1); \; \prismcomment{// increase buffer occupation}$} \\

\mbox{$ \;  \; [\prismident{toc}] \; (!(\prismident{m1}{=}1 \; \& \; \prismident{b0}{>}0 \; \& \; \prismident{b1}{<}\prismident{n1}) \; \& \; (\prismident{m2}{=}1 \; \& \; \prismident{b1}{>}0 \; \& \; \prismident{b2}{<}\prismident{n2})) \; \rightarrow$} \\ \; \; \mbox{$1:(\prismident{b1'}{=}\prismident{b1}-1); \; \prismcomment{// decrease buffer occupation}$} \\

\mbox{$ \;  \; [\prismident{toc}] \; ( \; (!(\prismident{m1}{=}1 \; \& \; \prismident{b0}{>}0 \; \& \; \prismident{b1}{<}\prismident{n1}) \; \& \; !(\prismident{m2}{=}1 \; \& \; \prismident{b1}{>}0 \; \& \; \prismident{b2}{<}\prismident{n2})) \; |$} \\

\mbox{$ \;  \;  \;  \;  \;  \;  \;  \;  \;  \;  \; ((\prismident{m1}{=}1 \; \& \; \prismident{b0}{>}0 \; \& \; \prismident{b1}{<}\prismident{n1}) \; \& \; (\prismident{m2}{=}1 \; \& \; \prismident{b1}{>}0 \; \& \; \prismident{b2}{<}\prismident{n2})) \; ) \; \rightarrow$} \\ \; \; \; \; \; \; \; \; \;  \mbox{$1:(\prismident{b1'}{=}\prismident{b1}); \; \prismcomment{// buffer unchanged}$} \\

\mbox{$\prismkeyword{endmodule}$} \\

\mbox{$\prismkeyword{module} \; \prismident{M2}{=} \; \prismident{M1}[\prismident{m1}{=}\prismident{m2}, \; \prismident{b0}{=}\prismident{b1}, \; \prismident{b1}{=}\prismident{b2}, \; \prismident{p1}{=}\prismident{p2}, \; \prismident{r1}{=}\prismident{r2}, \; \prismident{n1}{=}\prismident{n2},$} \; \\ \; \; 

\mbox{$\prismident{m1init}{=}\prismident{m2init}]$} \; \\ \mbox{$\prismkeyword{endmodule} \; $} \\

\mbox{$\prismkeyword{module} \; \prismident{B2}{=} \; \prismident{B1}[\prismident{b1}{=}\prismident{b2}, \; \prismident{m1}{=}\prismident{m2}, \; \prismident{m2}{=}\prismident{m3}, \; \prismident{b0}{=}\prismident{b1}, \; \prismident{b2}{=}\prismident{b3}, \; \prismident{n1}{=}\prismident{n2}, \; \prismident{n2}{=}\prismident{n3},$} \\ \; \; 

\mbox{$\prismident{b1init}{=}\prismident{b2init}]$} \; \\ 
\mbox{$\prismkeyword{endmodule} \; $} \\
\mbox{$\prismkeyword{module} \; \prismident{M3}{=} \; \prismident{M2}[\prismident{m2}{=}\prismident{m3}, \; \prismident{b1}{=}\prismident{b2}, \; \prismident{b2}{=}\prismident{b3}, \; \prismident{p2}{=}\prismident{p3}, \; \prismident{r2}{=}\prismident{r3}, \; \prismident{n2}{=}\prismident{n3},$} \; \\ \; \; \mbox{$\prismident{m2init}{=}\prismident{m3init}]$} \; \\ \mbox{$\prismkeyword{endmodule} \; $} 



\end{tabbing}
\end{minipage}}}
\end{center}
\medskip


==> prism_tex/guardedCommand.tex <==
\medskip
%\centering
\begin{center}
{%\scriptsize
\footnotesize
\fbox{\begin{minipage}{6in}
\begin{tabbing}
\mbox{$ \;  \; [\prismident{action\_name}] \; \prismkeyword{guard} \; \rightarrow \; \prismkeyword{probabilistic\_updates};$} 
\end{tabbing}
\end{minipage}}}
\end{center}


==> prism_tex/guardedCommandSynch.tex <==
\medskip
%\centering
\begin{center}
{%\scriptsize
\footnotesize
\fbox{\begin{minipage}{6in}
\begin{tabbing}
\mbox{$\prismkeyword{module} \; \prismident{M1} $} \\
\mbox{$ \;  \; [\prismident{action1}] \; \prismkeyword{guard1} \; \rightarrow \; \prismident{p$_1$}:(\prismkeyword{updt$_{1,1}$}) \; + ... + \; (\prismident{p$_n$}):(\prismkeyword{updt$_{n,1}$})$} \\
\mbox{$\prismkeyword{endmodule}$} \\

\mbox{$\prismkeyword{module} \; \prismident{M2} $} \\
\mbox{$ \;  \; [\prismident{action1}] \; \prismkeyword{guard2} \; \rightarrow \;  \prismident{q$_1$}:(\prismkeyword{updt$_{1,2}$}) \; + ... + \; (\prismident{q$_m$}):(\prismkeyword{updt$_{m,2}$})$} \\
\mbox{$\prismkeyword{endmodule}$} 
\end{tabbing}
\end{minipage}}}
\end{center}


==> prism_tex/probUpdates.tex <==
\medskip
%\centering
\begin{center}
{%\scriptsize
\footnotesize
\fbox{\begin{minipage}{6in}
\begin{tabbing}
\mbox{$ \;  \; \prismident{p$_1$}:(\prismkeyword{update$_1$}) \; + ... + \; (\prismident{p$_n$}):(\prismkeyword{update$_n$})$} 
\end{tabbing}
\end{minipage}}}
\end{center}
\medskip


==> prism_tex/probUpdatesSynch.tex <==
\medskip
%\centering
\begin{center}
{%\scriptsize
\footnotesize
\fbox{\begin{minipage}{6in}
\begin{tabbing}
\mbox{$ \;  \; \prismident{p$_1 q_1$}:(\prismkeyword{updt$_{1,1}$})\&(\prismkeyword{updt$_{1,2}$}) \; + ... + \; \prismident{p$_n$q$_m$}:(\prismkeyword{updt$_{n,1}$})\&(\prismkeyword{updt$_{m,2}$})$} 
\end{tabbing}
\end{minipage}}}
\end{center}
\medskip


==> prism_tex/toyExample1.tex <==
\medskip
%\centering
\begin{center}
{\scriptsize
%\footnotesize
\fbox{\begin{minipage}{6in}
\begin{tabbing}
\mbox{$\prismkeyword{dtmc}$} \\
\mbox{$\prismkeyword{const} \; \prismkeyword{double} \; \prismident{p1}{=}{0.01}; \;  \; \prismcomment{// fail probability  }$} \\
\mbox{$\prismkeyword{const} \; \prismkeyword{double} \; \prismident{r1}{=}0.1; \;  \; \prismcomment{// repair probability  }$} \\
\mbox{$\prismkeyword{const} \; \prismkeyword{int} \; \prismident{m1init}{=}1; \;  \; \prismcomment{// initial state  }$} \\
%\mbox{$$} \\

\mbox{$\prismkeyword{module} \; \prismident{M1} \; \prismcomment{// a faulty/repairable  machine}$} \\
\mbox{$ \;  \; \prismident{m1} \; : \; [0..1] \; \prismkeyword{init} \; \prismident{m1init};$} \\
\mbox{$ \;  \; [\prismident{fail}] \; \prismident{m1}{=}1 \;  \;  \; \rightarrow \; \prismident{p1}:(\prismident{m1'}  {=}  {0}) \; + \; (1-\prismident{p1}):(\prismident{m1'}{=}1);$} \\
\mbox{$ \;  \; [\prismident{repair}] \; \prismident{m1}{=}0 \;  \;  \; \rightarrow \; \prismident{r1}:(\prismident{m1'}{=}1) \; + \; (1-\prismident{r1}):(\prismident{m1'}{=}0); \;  \; $} \\
\mbox{$\prismkeyword{endmodule}$} 
\end{tabbing}
\end{minipage}}}
\end{center}
\medskip


==> prism_tex/toyExample2.tex <==
\medskip
%\centering
\begin{center}
{\scriptsize
%\footnotesize
\fbox{\begin{minipage}{6in}
\begin{tabbing}
\mbox{$\prismkeyword{dtmc}$} \\
\mbox{$\prismkeyword{const} \; \prismkeyword{double} \; \prismident{p1}{=}{0.01}; \;  \; \prismcomment{// fail probability  }$} \\
\mbox{$\prismkeyword{const} \; \prismkeyword{double} \; \prismident{r1}{=}0.1; \;  \; \prismcomment{// repair probability  }$} \\
\mbox{$\prismkeyword{const} \; \prismkeyword{int} \; \prismident{m1init}{=}1; \;  \; \prismcomment{// machine initial state }$} \\
\mbox{$\prismkeyword{const} \; \prismkeyword{int} \; \prismident{b1init}{=}0; \;  \; \prismcomment{// buffer initial state  }$} \\
\mbox{$\prismkeyword{const} \; \prismkeyword{int} \; \prismident{n1}{=}5; \;  \; \prismcomment{// buffer size  }$} \\


\mbox{$\prismkeyword{module} \; \prismident{M1} \; \prismcomment{// a faulty/repairable  machine}$} \\
\mbox{$ \;  \; \prismident{m1} \; : \; [0..1] \; \prismkeyword{init} \; \prismident{m1init};$} \\
\mbox{$ \;  \; [\prismident{tic}] \; \prismident{m1}{=}1 \;  \;  \; \rightarrow \; \prismident{p1}:(\prismident{m1'}  {=}  {0}) \; + \; (1-\prismident{p1}):(\prismident{m1'}{=}1);$} \\
\mbox{$ \;  \; [\prismident{tic}] \; \prismident{m1}{=}0 \;  \;  \; \rightarrow \; \prismident{r1}:(\prismident{m1'}{=}1) \; + \; (1-\prismident{r1}):(\prismident{m1'}{=}0); \;  \; $} \\
\mbox{$\prismkeyword{endmodule}$} \\

\mbox{$\prismkeyword{module} \; \prismident{B1} \; \prismcomment{// a finite-size buffer}$} \\
\mbox{$ \;  \; \prismident{b1} \; : \; [0..\prismident{n1}] \; \prismkeyword{init} \; \prismident{b1init};$} \\
\mbox{$ \;  \; [\prismident{tic}] \; \prismident{m1}{=}1 \;  \;  \; \rightarrow \; {1}:(\prismident{b1'}  {=}  {min(b1+1,n1)});$} \\
\mbox{$ \;  \; [\prismident{tic}] \; \prismident{m1}{=}0 \;  \;  \; \rightarrow \; {1}:(\prismident{b1'}  {=}  {max(b1-1,0)});$} \\
\mbox{$\prismkeyword{endmodule}$} 
\end{tabbing}
\end{minipage}}}
\end{center}
\medskip


==> prism_tex/update.tex <==
\medskip
%\centering
\begin{center}
{%\scriptsize
\footnotesize
\fbox{\begin{minipage}{6in}
\begin{tabbing}
\mbox{$ \;  \; (\prismident{var$_1$'} \; {=} \;  \; \prismkeyword{exp$_1$}) \& ... \& (\prismident{var$_m$'} \; {=} \;  \; \prismkeyword{exp$_m$})$} 
\end{tabbing}
\end{minipage}}}
\end{center}
\medskip


==> sections/methods.tex <==
%%%% SECTION %%%%%%%%%%%%
\section{HASL based performance analysis of production lines}
\label{sec:methods}

